SpatialAnt: Autonomous Zero-Shot Robot Navigation via Active Scene Reconstruction and Visual Anticipation

Vision-and-Language Navigation (VLN) has recently benefited from Multimodal Large Language Models (MLLMs), enabling zero-shot navigation. While recent exploration-based zero-shot methods have shown promising results by leveraging global scene priors, they rely on high-quality human-crafted scene reconstructions, which are impractical for real-world robot deployment. When encountering an unseen environment, a robot should build its own priors through pre-exploration. However, these self-built reconstructions are inevitably incomplete and noisy, which severely degrade methods that depend on high-quality scene reconstructions. To address these issues, we propose SpatialAnt, a zero-shot navigation framework designed to bridge the gap between imperfect self-reconstructions and robust execution. SpatialAnt introduces a physical grounding strategy to recover the absolute metric scale for monocular-based reconstructions. Furthermore, rather than treating the noisy self-reconstructed scenes as absolute spatial references, we propose a novel visual anticipation mechanism. This mechanism leverages the noisy point clouds to render future observations, enabling the agent to perform counterfactual reasoning and prune paths that contradict human instructions. Extensive experiments in both simulated and real-world environments demonstrate that SpatialAnt significantly outperforms existing zero-shot methods. We achieve a 66% Success Rate (SR) on R2R-CE and 50.8% SR on RxR-CE benchmarks. Physical deployment on a Hello Robot further confirms the efficiency and efficacy of our framework, achieving a 52% SR in challenging real-world settings.

==> tables/debug.tex <==

\begin{figure}[t] % 注意这里去掉了 *，限制在单栏内
    \centering
    \centering
\small
\captionsetup{skip=2pt}
\setlength{\tabcolsep}{5pt}
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{3pt}

    % ==========================================
    % 上半部分：表格 (占满这一栏的宽度)
    % ==========================================
    % \begin{minipage}{\linewidth}
        \small
        % \captionsetup{type=table} % 强行声明这里是 Table 编号
        \caption{\textbf{Trigger Conditions vs. Performance:} Comparison of various dialogue trigger strategies, evaluations are conducted on the same 100 sampled episodes of R2R-CE as in Tab.~\ref{tab:continuous_main}.}
        \label{tab:ablation_triggers}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{l ccc c}
        \toprule
        \textbf{Trigger Strategy} & \textbf{SR ($\uparrow$)} & \textbf{SPL ($\uparrow$)} & \textbf{Count} & \textbf{Rate} \\
        \midrule
        None (Baseline)     & 48.8 & 41.8 & 0.00 & 0.0\% \\
        Repeat ($\mathcal{C}_{\mathrm{rep}}$) & 57.0 & 45.1 & 88 & 4.74\% \\
        \rowcolor{gray!10}
        \textbf{Deviation ($\mathcal{C}_{\mathrm{away}}$)} & \textbf{66.0} & \textbf{49.4} & 279 & 15.0\% \\
        Hybrid (Both)       & 54.0 & 44.5 & 477 & 23.1\% \\
        Periodic ($k=5$)    & 63.0 & 46.5 & 113 & 10.2\% \\
        \midrule
        Human-in-the-Loop   & 74.5 & 61.2 & 105 & 9.8\% \\
        \bottomrule
        \end{tabular}
        }
    % \end{minipage}
    
    % \vspace{5mm} % 在表和图之间加上适当的垂直间距，让它们看起来不拥挤
    
    % % ==========================================
    % % 下半部分：折线图 (占满这一栏的宽度)
    % % ==========================================
    % \begin{minipage}{\linewidth}
    %     \centering
    %     \captionsetup{type=figure} % 声明恢复回 Figure 编号
    %     \includegraphics[width=\linewidth]{figs/periodic_frequency.pdf} 
    %     % \vspace{-2mm} % 微调图和Caption的距离
    %     \caption{\textbf{Impact of Intervention Frequency on Different Agents:} Comparison of navigation performance under varying periodic intervention intervals ($k$). The evaluation contrasts the performance trends of a vanilla baseline agent (NavGPT) with a more complex agent architecture (GTA).}
    %     \label{fig:periodic_interval}
    % \end{minipage}
    
\end{figure}
